Can Large Language Models Trade? Testing Financial Theories with LLM Agents in Market Simulations

This paper presents a realistic simulated stock market where large language models (LLMs) act as heterogeneous competing trading agents. The open-source framework incorporates a persistent order book with market and limit orders, partial fills, dividends, and equilibrium clearing alongside agents with varied strategies, information sets, and endowments. Agents submit standardized decisions using structured outputs and function calls while expressing their reasoning in natural language. Three findings emerge: First, LLMs demonstrate consistent strategy adherence and can function as value investors, momentum traders, or market makers per their instructions. Second, market dynamics exhibit features of real financial markets, including price discovery, bubbles, underreaction, and strategic liquidity provision. Third, the framework enables analysis of LLMs' responses to varying market conditions, similar to partial dependence plots in machine-learning interpretability. The framework allows simulating financial theories without closed-form solutions, creating experimental designs that would be costly with human participants, and establishing how prompts can generate correlated behaviors affecting market stability.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
[Broader implications and limitations]

==> sections/model.tex <==
\section{Theoretical Framework}
\label{sec:model}

While our framework ultimately relies on LLM agents operating through natural language, developing a formal theoretical model serves several purposes. First, it provides analytical structure for understanding and predicting agent behavior, allowing us to bridge the gap between traditional economic theory and LLM-based decision making. Second, it enables us to derive testable predictions about market outcomes, creating a systematic framework for validating whether LLM agents behave in economically meaningful ways. Third, it helps identify potential sources of market instability or inefficiency that might emerge from LLM trader interactions, informing both practical system design and regulatory policy.

The model we develop maintains sufficient mathematical precision to derive clear predictions while accommodating the unique characteristics of LLM agents. Rather than assuming explicit utility maximization, we model how trading strategies emerge from natural language prompts and reason about how these strategies interact to determine market outcomes. This hybrid approach - combining rigorous economic modeling with LLM-based decision making - provides new insights into how markets might function when populated by AI traders while maintaining connection to classical market microstructure theory.

\subsection{Market Structure}
We consider a finite-horizon market operating over the interval $[0,T]$. The market structure incorporates key features of modern electronic trading venues while maintaining analytical tractability. This section details the fundamental components of our market model, including order types, execution mechanisms, and price formation processes.

\subsubsection{Order Types and Execution Mechanism}
The market supports a dual-order system consisting of market and limit orders. Market orders provide immediate execution certainty at the best available price, while limit orders allow traders to specify execution prices but without guaranteed fills. This structure captures the fundamental tradeoff between execution certainty and price improvement that traders face in real markets.

Order execution follows a strict price-time priority rule, consistent with the majority of modern electronic markets. Under this mechanism, market orders receive immediate execution priority, while limit orders enter a queue based on their price level and submission time. When limit orders cross the spread (i.e., buy orders with prices at or above the best ask, or sell orders with prices at or below the best bid), they are automatically converted to market orders to ensure immediate execution.

The market operates in discrete rounds, with each round $t$ following a four-stage matching process:
\begin{enumerate}
\item First, the system processes cancellations of existing orders from active agents
\item Next, it executes any new market orders against available liquidity
\item Then, it adds new limit orders to the order book
\item Finally, it matches any crossing limit orders according to price-time priority
\end{enumerate}

The market clearing price $P_t$ at each round is determined by a standard mechanism:
\[P_t = \begin{cases}
P_\text{trade} & \text{if trades occur} \\
\frac{P_\text{bid} + P_\text{ask}}{2} & \text{if no trades}
\end{cases}\]
where $P_\text{trade}$ represents the last executed trade price, and $P_\text{bid}$ and $P_\text{ask}$ are the best bid and ask prices in the order book. This price formation process ensures continuous price discovery even in the absence of trades, while maintaining a clear connection to actual transaction prices when trading occurs.

\subsubsection{Dividend Process}
The traded asset generates a continuous dividend stream that follows a geometric Brownian motion, reflecting the standard modeling approach in financial economics. The dividend process evolves according to:
\[dD_t = \mu dt + \sigma_D dW_t\]
where $\mu$ represents the expected dividend growth rate, $\sigma_D$ captures dividend volatility, and $W_t$ is a standard Wiener process. This specification allows for both predictable growth through the drift term and random fluctuations through the diffusion term, providing a realistic model of dividend uncertainty.

\subsubsection{Asset Structure}
The asset's value structure combines both finite and continuous components. Specifically, investors receive a continuous dividend stream $D_t$ throughout the trading period and a terminal value $K$ at time $T$. This dual-component structure creates rich trading dynamics as agents must balance immediate dividend income against terminal value considerations in their trading decisions.

\subsubsection{Agent Endowments and Constraints}
Each agent $i$ enters the market with an initial endowment consisting of cash $C_{i,0}$ and shares $S_{i,0}$. To maintain market realism and prevent degenerate trading strategies, agents face two key constraints. First, a non-negative cash constraint ($C_{i,t} \geq 0$) prevents unlimited borrowing. Second, a short-selling constraint ($S_{i,t} \geq -\bar{S}$) limits agents' ability to take negative positions, where $\bar{S}$ represents the maximum allowed short position. These constraints ensure that trading strategies remain within economically reasonable bounds while still allowing for substantial trading flexibility.

\subsubsection{Fundamental Value}
The fundamental value of the asset at any time $t$ represents the present value of all future cash flows, combining both the terminal value and the dividend stream. Specifically, the fundamental value is calculated as:
\[V_t = K e^{-r(T-t)} + \int_t^T E[D_s]e^{-r(s-t)}ds\]
where $r$ represents the risk-free interest rate and $E[D_s]$ denotes the expected dividend at time $s$. The first term captures the discounted terminal value, while the integral term accounts for the continuous stream of expected future dividends, each appropriately discounted to present value.

\subsubsection{Parameter Calibration}
To facilitate clear analysis of trading behavior, we calibrate the model parameters $\{\mu, K, r, T\}$ to maintain a constant fundamental value throughout the trading period, such that $V_t = V^*$ for all $t \in [0,T]$. This stability is achieved by setting the dividend growth rate as:
\[\mu = rV^* - rK e^{-r(T-t)}\]
This calibration creates a stable benchmark against which to evaluate agent behavior, eliminating confounding effects from time-varying fundamentals and allowing us to focus on the strategic interactions between trading agents.

\subsection{LLM Decision Process}
The LLM trading agent integrates multiple information sources to form trading decisions. At each decision point, the agent processes four key components: a strategy template $\theta_i$ derived from its initial prompt, the current market state $S_t$, historical context $H_t$ consisting of past states, actions, and reasoning ($\{(S_k, a_k, R_k)\}_{k<t}$), and its natural language reasoning output $R_t$.

The agent's decision framework encompasses several key variables. The action space includes three possible decisions ($a_t \in \{\text{Buy}, \text{Sell}, \text{Hold}\}$), complemented by quantity decisions ($q_t$) and order type selection ($o_t \in \{\text{Market}, \text{Limit}\}$). Each agent operates according to its assigned strategy type $\theta_i$. The market state $S_t$ is represented by a comprehensive set of variables: current price ($P_t$), fundamental value ($V_t$), price changes ($\Delta P_t$), trading volume ($\text{Vol}_t$), inventory levels ($I_t$), and news signals ($N_t$).

This information processing results in a probabilistic distribution over possible actions, formally expressed as:
\[P(a_t, q_t, o_t|\theta_i, S_t, H_t) = \text{LLM}(\theta_i, S_t, H_t)\]

The agent's decision space can be characterized mathematically as:
\[\mathcal{D} = \{(a, q, o) \in \mathcal{A} \times \mathcal{Q} \times \mathcal{O} : \text{feasible}(a, q, o|\theta_i, S_t)\}\]
where feasibility is constrained by both explicit market rules and learned strategic behavior. While LLMs do not compute explicit probabilities in their decision-making process, their behavior can be approximated by a function mapping strategy and state to actions:
\[P(a_t, q_t, o_t|\theta_i, S_t) = g(\theta_i, S_t)\]

\subsection{Prompt-Based Strategy Formation}

A strategy $\theta_i$ emerges from three components:
\begin{enumerate}
\item Base prompt template $\pi_i^b$
\item Strategy-specific rules $\pi_i^s$
\item Context window $C_t$
\end{enumerate}

The prompt-to-strategy mapping can be formalized as:
\[\theta_i = g(\pi_i^b \oplus \pi_i^s, C_t)\]

where $\oplus$ represents prompt composition, $C_t = \{S_k, a_k, R_k\}_{k=t-w}^t$ is the context window of length $w$, and $g(\cdot)$ is the LLM's interpretation function.

For example, a value investor's strategy components are:
\begin{align*}
\pi_i^b &= \text{"You are a trading agent..."} \\
\pi_i^s &= \text{"Buy when price $<$ fundamental value..."} \\
C_t &= \text{Recent market states and actions}
\end{align*}

More formally, each strategy type's prompt structure can be decomposed as:
\[\pi_i = \{\pi_i^\text{role}, \pi_i^\text{constraints}, \pi_i^\text{objectives}, \pi_i^\text{rules}\}\]

where $\pi_i^\text{role}$ defines the agent's role, $\pi_i^\text{constraints}$ specifies trading restrictions, $\pi_i^\text{objectives}$ states optimization goals, and $\pi_i^\text{rules}$ provides decision heuristics. This decomposition ensures that each agent maintains consistent behavior aligned with its assigned trading strategy while retaining the flexibility to adapt to changing market conditions within its strategic framework.

\subsection{LLM Reasoning Process}

The decision-making process of the LLM unfolds in three distinct stages. First, during the Information Processing stage, the LLM synthesizes the current market state $S_t$, historical context $H_t$, and its strategy template $\theta_i$ to produce a processed market state $\hat{S}_t$. This is represented mathematically as:
\[\hat{S}_t = f_\text{process}(S_t, H_t, \theta_i)\]

Next, in the Strategy Application stage, the LLM applies its reasoning capabilities to the processed market state $\hat{S}_t$ and its strategy template $\theta_i$, generating a natural language reasoning output $R_t$:
\[R_t = f_\text{reason}(\hat{S}_t, \theta_i)\]

Finally, in the Decision Formation stage, the LLM uses the reasoning output $R_t$ to form a probabilistic distribution over possible actions, quantities, and order types:
\[P(a_t, q_t, o_t|R_t) = f_\text{decide}(R_t)\]

In this framework, $\hat{S}_t$ represents the processed market state, $R_t$ is the natural language reasoning, and $f_\text{process}, f_\text{reason}, f_\text{decide}$ are functions specific to the LLM's architecture.

The reasoning output $R_t$ itself can be decomposed into four components: observation ($O_t$), analysis ($A_t$), decision ($D_t$), and justification ($J_t$). This decomposition provides a structured approach to understanding how the LLM interprets and acts upon market information.

\subsection{Trade Formation}

\subsubsection{Quantity Decisions}
Each agent's desired trade quantity is determined by:
\[q_t = \max\{\min\{q^*(\theta_i, S_t), q_\text{max}\}, 0\}\]
where $q^*(\theta_i, S_t)$ is the desired trade size based on strategy and state, and $q_\text{max}$ is the position limit. This formulation ensures that trade quantities remain within feasible bounds while reflecting the agent's strategic preferences and market conditions. The nested max-min structure enforces both non-negative quantities and maximum position constraints, preventing degenerate trading behavior while maintaining strategic flexibility.

\subsection{LLM-Induced Strategy Functions}

These strategy functions emerge from natural language prompts rather than explicit programming. While LLMs do not calculate explicit parameters, their natural language reasoning effectively implements similar decision boundaries. For analytical tractability, we can approximate each agent type's behavior with a specific functional form $g_\theta$:

\subsubsection{Value Investor}
$g_\text{value} = f(P_t/V_t)$ with prompt-induced parameters $\alpha, \beta$:
\begin{itemize}
\item Buy if $P_t/V_t < 1 - \alpha$ 
\item Sell if $P_t/V_t > 1 + \alpha$
\item Market if $|P_t/V_t - 1| > \beta$
\end{itemize}

\subsubsection{Momentum Trader}
$g_\text{momentum} = f(\Delta P_t, \Delta \text{Vol}_t)$ with parameters $\gamma, \sigma_t$:
\begin{itemize}
\item Buy if $\Delta P_t > 0$ and $\Delta \text{Vol}_t > 0$
\item Sell if $\Delta P_t < 0$ or $\Delta \text{Vol}_t < 0$
\item Market if $|\Delta P_t| > \sigma_t$
\end{itemize}

\subsubsection{Market Maker}
$g_\text{maker} = f(I_t - I^*, P_t - \bar{P}_t)$ with parameters $\delta, \lambda$:
\begin{itemize}
\item Buy if $I_t < I^*$ and $P_t < \bar{P}_t$
\item Sell if $I_t > I^*$ and $P_t > \bar{P}_t$
\item Limit by default, Market if $|I_t - I^*| > \delta$
\end{itemize}

\subsubsection{Contrarian Trader}
$g_\text{contrarian} = f((P_t - \bar{P}_t)/\sigma_t, \text{Vol}_t)$ with parameters $\eta, \mu$:
\begin{itemize}
\item Buy if $(P_t - \bar{P}_t)/\sigma_t < -\eta$
\item Sell if $(P_t - \bar{P}_t)/\sigma_t > \eta$
\item Market if $|(P_t - \bar{P}_t)/\sigma_t| > \mu$
\end{itemize}

\subsubsection{News Trader}
$g_\text{news} = f(N_t, P_t - \bar{P}_t)$ with parameters $\nu, \xi$:
\begin{itemize}
\item Buy if $N_t > 0$ and $P_t < \bar{P}_t$
\item Sell if $N_t < 0$ or $P_t > \bar{P}_t + \xi|N_t|$
\item Market if $|N_t| > \nu$
\end{itemize}

\subsubsection{Optimistic Trader}
$g_\text{optimistic} = f(P_t, 10V_t)$ with parameter $\kappa$:
\begin{itemize}
\item Buy if $P_t < 10V_t - \kappa$
\item Sell if $P_t > 10V_t + \kappa$
\item Market by default
\end{itemize}

\subsubsection{Speculator}
$g_\text{spec} = f(E[\Delta P_t])$ with parameters $\psi, \omega$:
\begin{itemize}
\item Buy if $E[\Delta P_t] > \psi$
\item Sell if $E[\Delta P_t] < -\psi$
\item Market if $|E[\Delta P_t]| > \omega$
\end{itemize}

where $\bar{P}_t$ is the moving average price, $I^*$ is the target inventory level, $\sigma_t$ is the price volatility, and $E[\Delta P_t]$ is the expected price change. Parameters ($\alpha, \beta, \gamma, \delta, \eta, \nu, \kappa, \psi, \omega$) represent the implicit thresholds that emerge from the LLM's interpretation of strategy-specific prompts. This formalization, while an approximation of the complex reasoning process within LLMs, provides sufficient mathematical structure for theoretical analysis while maintaining fidelity to the underlying natural language implementation.

\subsection{Linear Approximations of Strategy Functions}

While the LLM agents operate through natural language reasoning, their behavior can be approximated using linear decision rules for analytical tractability. These approximations capture the first-order effects of key state variables on trading decisions.

\subsubsection{General Form}
Each agent's trading decision can be approximated as a linear function:
\[q_t = \beta_0 + \sum_i \beta_i x_{i,t}\]
where $q_t$ is the desired trade quantity (positive for buy, negative for sell), $\beta_i$ are strategy-specific coefficients, and $x_{i,t}$ are state variables.

\subsubsection{Strategy-Specific Approximations}

For value investors, trading quantity is proportional to the relative price-value discrepancy:
\[q_t = \beta_v \left(\frac{V_t - P_t}{V_t}\right) + \epsilon_t\]
where $\beta_v > 0$ reflects sensitivity to value-price discrepancy.

Momentum traders respond to both price and volume changes:
\[q_t = \beta_p \Delta P_t + \beta_v \Delta \text{Vol}_t + \epsilon_t\]
where $\beta_p, \beta_v > 0$ capture price and volume momentum sensitivity.

Market makers balance inventory management with price reversion:
\[q_t = \beta_i(I^* - I_t) + \beta_p(P_t - \bar{P}_t) + \epsilon_t\]
where $\beta_i > 0$ and $\beta_p < 0$ reflect inventory and price reversion goals.

Contrarian traders act against normalized price deviations:
\[q_t = -\beta_z \left(\frac{P_t - \bar{P}_t}{\sigma_t}\right) + \epsilon_t\]
where $\beta_z > 0$ captures mean reversion strength.

News traders combine signal response with price adjustment:
\[q_t = \beta_n N_t + \beta_p(P_t - \bar{P}_t) + \epsilon_t\]
where $\beta_n > 0$ and $\beta_p < 0$ reflect news sensitivity and price adjustment.

Optimistic traders pursue aggressive value targets:
\[q_t = \beta_o(10V_t - P_t) + \epsilon_t\]
where $\beta_o > 0$ reflects optimistic value sensitivity.

Speculators trade on expected price movements:
\[q_t = \beta_e E[\Delta P_t] + \epsilon_t\]
where $\beta_e > 0$ captures expected price change sensitivity.

\subsubsection{Order Type Selection}
The probability of selecting a market order can be modeled as:
\[\text{Pr}(\text{Market}) = \Phi(\gamma_0 + \gamma_1|q_t| + \gamma_2|\Delta P_t|)\]
where $\Phi(\cdot)$ is the standard normal CDF, $\gamma_1 > 0$ captures urgency based on trade size, and $\gamma_2 > 0$ reflects price movement sensitivity.

\subsubsection{Empirical Estimation}
These coefficients can be estimated from LLM trading data using standard linear regression:
\[\hat{\beta} = (X'X)^{-1}X'q\]
where $X$ is the matrix of state variables, $q$ is the vector of trade quantities, and $\hat{\beta}$ are the estimated strategy coefficients. This empirical approach allows us to quantify how closely the LLM agents adhere to their intended trading strategies and measure the relative importance of different state variables in their decision-making process.

\subsection{Prompt-Based Adaptation}

Unlike traditional models with fixed parameters, LLM agents can adapt their decision thresholds ($\alpha, \beta, \gamma$, etc.) based on market conditions while maintaining strategic consistency. This adaptation process can be modeled as:

\[\theta_{i,t+1} = h(\theta_{i,t}, S_t, R_t)\]

where $\theta_{i,t}$ represents the agent's current strategy parameters, $S_t$ is the market state, and $R_t$ is the reasoning output from the LLM. This dynamic adaptation allows agents to respond to changing market conditions while maintaining their fundamental strategic orientation.

\subsection{Market Clearing and Equilibrium}

\subsubsection{Market Clearing}
The market clears through the standard conditions:
\begin{align*}
\sum_i q_{i,t} &= 0 \\
\sum_i S_{i,t} &= \bar{S}_\text{total}
\end{align*}

where $\bar{S}_\text{total}$ is the total supply of shares. These conditions ensure that trading remains a zero-sum game in terms of quantity and that the total number of shares in the market remains constant.

\subsubsection{Wealth Evolution}
Agent wealth evolves according to:
\[W_{i,t} = C_{i,t} + S_{i,t}P_t + \int_0^t S_{i,s}D_s ds\]

This formulation captures all components of an agent's wealth: current cash holdings ($C_{i,t}$), the market value of their current position ($S_{i,t}P_t$), and the accumulated dividend income from their historical positions ($\int_0^t S_{i,s}D_s ds$).

\subsubsection{Equilibrium Definition}
An equilibrium in this market model consists of three main components: the price process $\{P_t\}_{t=0}^T$, the trading strategies $\{q_{i,t}\}_{i,t}$, and the holdings $\{S_{i,t}, C_{i,t}\}_{i,t}$. 

For an equilibrium to exist, several conditions must be satisfied. First, given the price $P_t$, each agent's strategy must maximize their expected utility while adhering to certain constraints. These include a budget constraint ensuring non-negative cash holdings ($C_{i,t} \geq 0$), position limits preventing excessive short-selling ($S_{i,t} \geq -\bar{S}$), and strategy consistency where the trading decision $q_{i,t}$ aligns with the agent's strategy function $g_{\theta_i}(S_t)$. 

Second, markets must clear at all times, meaning the total quantity of trades sums to zero, and the total supply of shares remains constant. Lastly, all agents must maintain solvency, ensuring their wealth $W_{i,t}$ is non-negative.

While traditional equilibrium concepts assume explicit utility maximization, LLM agents implicitly optimize through their strategy-specific prompts and natural language reasoning. This creates a novel form of equilibrium where optimal behavior emerges from prompt interpretation rather than mathematical optimization.

\subsection{Testable Predictions}

Our framework yields several quantitative predictions:

\subsubsection{Strategy Consistency}
Agents maintain consistent behavior within their strategy type:
\[\text{Var}(a_t|\theta_i) < \text{Var}(a_t)\]
\[\text{Cov}(a_t, a_{t'}|\theta_i) > 0\]
These conditions indicate that trading decisions exhibit lower variance when conditioned on strategy type, and actions are positively correlated across time within the same strategy.

\subsubsection{Strategy Differentiation}
Different strategies produce systematically different trading patterns:
\[E[q_t|\theta_i] \neq E[q_t|\theta_j] \quad \text{for } i \neq j\]
This inequality demonstrates that trading behavior varies systematically across strategy types, with each strategy generating distinct patterns of market activity.

\subsubsection{Price Impact}
The price impact of trades varies by strategy type:
\[\frac{\partial P_t}{\partial q_t} = \lambda + f(\theta_i)\]
where $f(\theta_i)$ captures strategy-specific price effects. This relationship suggests that market impact is not uniform across strategies but rather depends on the strategic orientation of the trading agent, reflecting differences in how various strategies are perceived and interpreted by the market.

\subsubsection{Empirical Tests}
These predictions can be tested through various empirical methods. First, time series analysis of trading decisions within strategy types can reveal consistency over time. Second, cross-sectional comparison of trading patterns across different strategies can highlight systematic differences. Third, event study analysis of price movements following trades can assess the impact of specific strategies on market prices. Finally, semantic analysis of LLM reasoning outputs $R_t$ can provide insights into the decision-making process. The key innovation is that these patterns emerge from natural language prompts rather than explicit programming, while maintaining mathematical regularity sufficient for empirical testing.

\subsubsection{Reasoning Consistency}
The semantic similarity of reasoning outputs $R_t$ should be higher within strategy types:
\[\text{sim}(R_t, R_{t'}|\theta_i) > \text{sim}(R_t, R_{t'}|\theta_i \neq \theta_j)\]
where $\text{sim}(\cdot,\cdot)$ is a semantic similarity measure. This suggests that agents with the same strategy type produce more consistent reasoning outputs compared to those with different strategies.

\subsection{Strategy Validation Framework}

The validation framework addresses three key questions: Does the agent maintain intended behavior (Strategy Fidelity)? Are choices economically rational (Decision Quality)? Is the logic sound and consistent (Reasoning Validity)?

We define three key validation metrics:

1. Strategy Consistency:
\[\text{SC}(\theta_i) = \frac{1}{T}\sum_{t=1}^T \text{sim}(R_t, E[R|\theta_i])\]

2. Decision Coherence:
\[\text{DC}(\theta_i) = \text{Cor}(D_t, D_{t+1}|\theta_i)\]

3. Reasoning Quality:
\[\text{RQ}(\theta_i) = \frac{1}{T}\sum_{t=1}^T \text{quality}(J_t|\theta_i, S_t)\]

where $\text{sim}(\cdot,\cdot)$ measures semantic similarity, $\text{Cor}(\cdot,\cdot)$ measures decision correlation, and $\text{quality}(\cdot)$ evaluates reasoning validity. A strategy is considered valid if it meets predetermined thresholds for these metrics:
\begin{align*}
\text{SC}(\theta_i) &\geq \alpha \\
\text{DC}(\theta_i) &\geq \beta \\
\text{RQ}(\theta_i) &\geq \gamma
\end{align*}

for predetermined thresholds $\alpha, \beta, \gamma$.








==> sections/reasoning_samples.tex <==
\subsection{Sample Agent Reasoning}

This section provides representative samples of agent reasoning, demonstrating how different 
agent types process market information and justify their trading decisions. Each sample includes 
the agent type, their decision, and their detailed reasoning.

The reasoning patterns demonstrate clear differentiation across agent types, reflecting their distinct
trading philosophies and decision frameworks. Value Investors consistently reference price-to-fundamental
ratios and historical averages, maintaining a disciplined focus on valuation metrics. Contrarian Traders
emphasize market sentiment and potential reversals, frequently citing excessive optimism or pessimism
in their decision-making. Optimistic agents demonstrate forward-looking perspectives, often discussing
price convergence to higher fundamental values while maintaining consistent bullish interpretations of
market conditions. These patterns reveal how different strategic frameworks lead to systematically
different interpretations of the same market data.



\subsubsection{Contrarian Trader}
\begin{quote}
\textbf{Round 8, Decision: Sell, OrderType.MARKET, Quantity: 75}

The current price of \$106.15 is significantly above the best estimate of fundamental value at \$28.00, indicating excessive optimism or overbuying in the market. The price-to-fundamental ratio is also higher than the historical average, suggesting unsustainable pricing. Additionally, there are no buy or sell orders, which may point to market indecision at this price level. Thus, i believe there is an opportunity to profit by selling at this inflated price.
\end{quote}

\subsubsection{Optimistic}
\begin{quote}
\textbf{Round 16, Decision: Buy, OrderType.MARKET, Quantity: 50}

The current price of \$114.95 is still significantly undervalued compared to my assessment of the fundamental value, which i believe should be \$280.00 (10x the estimated value). I see a strong potential for convergence to a higher price, so i will buy more shares to benefit from this expected increase. Since there are currently no orders in the market, i will place a market order for immediate execution.
\end{quote}

\subsubsection{Value Investor}
\begin{quote}
\textbf{Round 16, Decision: Hold}

The current price of \$114.95 is significantly above the fundamental value of \$28.00, resulting in a price/fundamental ratio of 4.11, which is also above the historical average of 3.83. This indicates that the asset is overvalued. According to my trading strategy, i should sell assets that are overvalued. However, there are no current sell orders in the order book, indicating a lack of market activity. Given that i currently hold zero shares, i'm unable to sell. Therefore, the decision is to hold, as there are no clear value opportunities for buying or selling right now.
\end{quote}

==> sections/results.tex <==
\section{Results}
\label{sec:results}

Our analysis reveals three key findings about the capabilities of LLM-based trading agents. First, we demonstrate that LLM agents exhibit consistent understanding of market mechanics and maintain coherent trading strategies. Through detailed analysis of agent decision logs and trading patterns, we find that agents reliably execute their assigned strategies while providing clear, contextually appropriate reasoning for their decisions. Value investors consistently reference fundamental prices in their decisions, while momentum traders demonstrate attention to price trends and volume patterns. This strategic consistency persists across varying market conditions and price regimes.

Second, our results show that LLM agents effectively contribute to price discovery and liquidity provision. Market maker agents maintain reasonable bid-ask spreads and actively manage their inventory positions, while value investors help anchor prices to fundamental values through their trading activities. Analysis of order book dynamics reveals that agents collectively maintain market depth and respond to liquidity demands. The interaction between different agent types creates realistic market dynamics, with prices generally tracking fundamental values while exhibiting plausible short-term deviations.

Third, we find evidence of sophisticated adaptation to changing market conditions while agents maintain their core strategic objectives. When faced with significant price movements or changes in fundamental values, agents adjust their trading behavior appropriately while remaining consistent with their assigned strategies. For instance, market makers widen spreads during periods of high volatility, and contrarian traders increase their activity during periods of extreme price movements. This adaptive behavior emerges naturally from the agents' LLM-based decision-making process rather than through explicit programming.

\subsection{Strategy Heterogeneity and Behavioral Consistency}
Our analysis reveals distinct behavioral patterns across agent types, demonstrating that LLM agents maintain consistent and differentiated trading strategies through prompt engineering alone. Value Investors exhibit highly conservative behavior, with only 2.1\% of their decisions being buy orders in our observation period. This conservative stance manifests not only in direction but also in execution style, with Value Investors using market orders in only 26.4\% of their trades, preferring more price-sensitive limit orders. Their trading frequency averages 2.0 trades per round, reflecting a deliberate and measured approach to market participation.

In contrast, Contrarian Traders demonstrate more balanced directional exposure, with 34.2\% of their decisions being buy orders, consistent with their mandate to trade against market extremes. These agents show higher trading activity, averaging 5.4 trades per round, and predominantly use market orders (82.5\%) to execute their counter-trend strategies. This higher trading frequency and market order usage suggests more opportunistic behavior in response to market movements.

Optimistic agents exhibit the most aggressive buying behavior, with 91.4\% of their decisions being buy orders, aligned with their belief in higher fundamental values. These agents are the most active, averaging 6.8 trades per round, and show strong preference for market orders (91.4\%), indicating high conviction in their positive outlook. Their behavior demonstrates that LLM agents can maintain consistent biases while still engaging actively with market conditions.

Analysis of agent reasoning provides further evidence of strategy adherence. Value-related keywords appear frequently across all agent types (averaging 3.74 mentions per decision for Value Investors), reflecting the high price-to-fundamental ratios observed during the trading period. However, agent-specific language patterns emerge clearly: Contrarian Traders show the highest usage of contrarian-strategy keywords (0.38 mentions per decision), while Optimistic agents consistently reference growth and upside potential (0.84 optimistic keywords per decision).

Price sensitivity analysis reveals that Value Investors maintain the largest spread between their buy and sell decisions relative to the price-fundamental ratio (buying at average P/F of 1.00, selling at 3.68), while Contrarian and Optimistic traders show more compressed ranges. This pattern demonstrates that different agent types systematically vary in their responses to market conditions while maintaining consistency with their assigned strategies.

\input{sections/reasoning_samples}



\subsection{Linguistic Analysis and Reasoning Patterns}

Topic modeling analysis reveals four distinct reasoning patterns in agent decision-making, each associated with different trading behaviors and agent types. The first topic, dominated by terms such as "overvalued," "fundamental," and "price," represents classical value-based reasoning. This topic appears in 89.3\% of Value Investor decisions but rarely in other agent types' reasoning, demonstrating strong adherence to their assigned strategy. The quantitative focus of this topic is evident in frequent references to specific ratios and price levels.

The second topic, characterized by terms like "converge," "believe," and references to price targets (e.g., "280"), captures forward-looking price expectations. This topic appears in 78.6\% of Optimistic agent decisions, aligning with their belief in higher fundamental values. The language in this topic cluster shows more certainty and conviction, with terms expressing belief and future price movements rather than current market conditions.

The third topic, featuring terms such as "excessive," "optimism," and "market shows," represents contrarian market analysis. This topic dominates Contrarian Trader reasoning (95.0\% of their decisions) and includes terms related to market sentiment and overreaction. The high concentration of this topic in Contrarian Trader decisions demonstrates their consistent focus on market psychology and extreme conditions.

The fourth topic focuses on execution mechanics, with terms like "market order," "bids," and "asks" appearing frequently. This topic appears across all agent types but with varying frequency (21.4\% for Optimistic agents, 5.0\% for Value Investors), suggesting different emphases on execution strategy. Notably, this topic correlates with higher market order usage and appears more frequently in decisions involving larger trade sizes.

Analysis of price patterns within topics reveals systematic relationships between reasoning and trading behavior. Topic 1 (optimistic outlook) shows the highest buy ratio (88.5\%) and moderate price-to-fundamental ratios, while Topic 0 (value-based reasoning) shows the lowest buy ratio (1.6\%) and appears at lower price-to-fundamental ratios. This alignment between topic distribution and trading patterns suggests that LLM agents maintain consistent relationships between their reasoning and actions.

These results demonstrate that LLM agents develop distinct linguistic patterns that align with their assigned strategies while maintaining internal consistency between their reasoning and trading decisions. The emergence of clear topic specialization across agent types, combined with systematic relationships between topics and trading patterns, suggests that LLM agents can maintain coherent decision-making frameworks that bridge qualitative reasoning and quantitative action.

\subsection{Semantic Consistency and Decision Coherence}

Semantic consistency measures the coherence and stability of an agent's reasoning across different decisions. We quantify this by embedding each reasoning text into a high-dimensional vector using a pre-trained sentence transformer model. By calculating the average pairwise cosine similarity of these vectors for each agent type, we obtain a semantic consistency score. This score reflects how consistently an agent applies its strategic reasoning framework, despite variations in market conditions.

Our analysis reveals high semantic consistency across all agent types, with Value Investors demonstrating the highest consistency (0.771), followed by Contrarian Traders (0.753) and Optimistic agents (0.741). These scores indicate that agents maintain coherent reasoning frameworks while adapting to changing market conditions. The high consistency scores suggest that LLM agents can effectively bridge qualitative reasoning with quantitative action, maintaining stable decision-making frameworks that align with their assigned strategies.

The semantic patterns show interesting variations across different market contexts. Value Investors exhibit the most formulaic reasoning, consistently referencing price-to-fundamental ratios (3.74 value-related keywords per decision) and maintaining strict decision criteria. This consistency manifests in both their reasoning and behavior, with the lowest buy ratio (0.021) and market order usage (0.264).

Contrarian Traders show a more nuanced pattern, balancing multiple semantic themes in their reasoning. While they frequently reference value concepts (2.81 value-related keywords per decision), they also incorporate contrarian indicators (0.383 contrarian keywords) and market sentiment analysis. This broader semantic scope aligns with their more balanced trading approach, evidenced by a moderate buy ratio (0.342) and higher trading frequency (5.4 trades per round).

Optimistic agents demonstrate an interesting linguistic pattern, frequently incorporating both optimistic (0.843 keywords per decision) and value-related concepts (2.407 keywords) in their reasoning. However, they reframe value metrics through an optimistic lens, as evidenced by Topic 1's emphasis on price convergence and future expectations. This optimistic reframing corresponds with their high buy ratio (0.914) and market order usage (0.914).

The topic distribution analysis reveals clear specialization in reasoning frameworks. Value Investors concentrate 89.3\% of their decisions in Topic 0 (fundamental analysis), while Contrarian Traders focus 95.0\% in Topic 2 (market sentiment), and Optimistic agents favor Topic 1 (price convergence) at 78.6\%. This topic specialization, combined with high semantic consistency scores, suggests that LLM agents develop stable, strategy-specific frameworks for market analysis.

Notably, all agent types show some presence of Topic 3 (execution mechanics), but with varying frequencies (5.0\% to 21.4\%), suggesting a shared understanding of market microstructure that complements their primary strategic focus. This layered approach to reasoning—combining strategy-specific analysis with practical trading considerations—demonstrates sophisticated decision-making capabilities in LLM agents.

\subsection{Market Efficiency and Trading Activity}

Our analysis reveals complex dynamics in price discovery and market efficiency. The market exhibits substantial initial deviation from fundamental values, with the price-to-fundamental ratio starting at 3.57. This overvaluation gradually corrects over the trading period, ending at 1.01, demonstrating the market's eventual convergence toward fundamental values. The correction process shows moderate volatility (0.178), suggesting orderly price adjustment rather than dramatic corrections.

Trading activity demonstrates consistent market engagement, with an average of 3.0 trades per round and mean volume of 20.3 units. The average trade size of 6.77 units indicates meaningful position-taking by market participants. Total trading activity accumulates to 406 units across 60 trades, suggesting sufficient liquidity for price discovery. This trading intensity, combined with the directional movement in prices toward fundamental values, indicates active and effective price discovery mechanisms.

The market's price efficiency metrics reveal both strengths and limitations in the price discovery process. While the market successfully moves prices toward fundamental values (P/F ratio change of -2.56), the average deviation from fundamental value remains substantial at 2.60. The range of price-to-fundamental ratios (min: 1.00, max: 4.23, std: 0.91) suggests periods of significant mispricing before correction. This pattern aligns with the observed agent behaviors, particularly the conservative stance of Value Investors (2.1\% buy ratio) and the more aggressive trading of Optimistic agents (91.4\% buy ratio).

The relationship between trading activity and price efficiency shows interesting patterns. Higher trading volumes tend to coincide with periods of price adjustment, suggesting that market participants actively trade when they identify mispricing opportunities. The average volume per round (20.3 units) provides sufficient depth for price discovery while avoiding excessive volatility, as evidenced by the moderate price volatility of 0.178.

These results suggest that LLM-based trading agents can collectively establish functioning market mechanisms, with prices responding to trading activity and gradually converging toward fundamental values. The persistence of some mispricing, despite active trading, indicates that market dynamics emerge from the complex interaction of different trading strategies rather than from simple arbitrage mechanisms.

\subsection{Agent Performance and Wealth Evolution}

Our analysis reveals striking differences in wealth accumulation across agent types, highlighting how different trading strategies performed in the experimental market environment. As shown in Figure~\ref{fig:agent_performance}, Optimistic agents dramatically outperformed other strategies, achieving a remarkable 3,732\% growth in dividend-adjusted wealth. This exceptional performance was driven by both aggressive position-taking and substantial dividend accumulation (8,859.20 in total dividends received).

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/agent_performance.png}
    \caption{Wealth evolution by agent type. Top: Total wealth including dividends shows exponential growth patterns, particularly for Optimistic agents. Bottom: Dividend-adjusted wealth reveals the underlying trading performance after controlling for dividend income. Note the logarithmic scale, highlighting the substantial differences in wealth accumulation rates across agent types.}
    \label{fig:agent_performance}
\end{figure}

Contrarian Traders demonstrated strong but more moderate performance, with dividend-adjusted wealth growth of 385.4\%. Their balanced trading approach and moderate dividend accumulation (890.40) suggest effective adaptation to market conditions while maintaining risk control. Value Investors, despite their conservative strategy, still achieved significant growth of 274.1\%, though their lower dividend accumulation (650.40) reflects their more cautious market participation.

These results suggest that in this market environment, characterized by initial overvaluation followed by correction (as shown in Section~\ref{sec:results}), optimistic trading strategies proved surprisingly effective. However, the substantial performance differences between agent types demonstrate that strategy selection significantly impacts trading outcomes, even when all agents operate with the same underlying LLM decision-making framework.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/market_efficiency.png}
    \caption{Market efficiency metrics over time. Top left: Price vs Fundamental Value shows the convergence of market prices toward fundamental value. Top right: Price/Fundamental Ratio demonstrates the correction of initial overvaluation. Bottom left: Trading Volume indicates market activity levels. Bottom right: Number of Trades and Average Trade Size reveals trading patterns and market depth.}
    \label{fig:market_efficiency}
\end{figure}



==> tables/results_tables.tex <==
% Trading Behavior Patterns
\begin{table}[ht]
\centering
\caption{Trading Behavior Patterns by Agent Type}
\label{tab:trading_behavior}
\begin{tabular}{lrrrr}
\toprule
 & buy\_ratio & market\_order\_ratio & avg\_quantity & trade\_frequency \\
\midrule
Value Investor & 0.02 & 0.26 & 12.11 & 2.00 \\
Contrarian Trader & 0.34 & 0.82 & 36.33 & 5.40 \\
Optimistic & 0.91 & 0.91 & 16.14 & 6.80 \\
\bottomrule
\end{tabular}
\end{table}


% Market Efficiency Metrics
\begin{table}[ht]
\centering
\caption{Market Efficiency Metrics}
\label{tab:market_efficiency}
\begin{tabular}{lr}
\toprule
 & Value \\
\midrule
Initial P/F Ratio & 3.57 \\
Final P/F Ratio & 1.01 \\
P/F Ratio Change & -2.56 \\
Total Trading Volume & 406.00 \\
Total Trades & 60.00 \\
Avg Trade Size & 6.77 \\
Price Volatility & 0.18 \\
Volume per Round & 20.30 \\
\bottomrule
\end{tabular}
\end{table}


% Agent Performance Summary
\begin{table}[ht]
\centering
\caption{Agent Performance Summary}
\label{tab:agent_performance}
\begin{tabular}{lrrrr}
\toprule
 & Initial Wealth & Final Wealth & Growth (\textbackslash \%) & Total Dividends \\
\midrule
Value Investor & 2,560.00 & 8,739.73 & 241.40 & 650.40 \\
Contrarian Trader & 2,560.00 & 11,495.21 & 349.03 & 890.40 \\
Optimistic & 2,560.00 & 89,515.65 & 3,396.70 & 8,859.20 \\
\bottomrule
\end{tabular}
\end{table}

